The Network Propensity Score: Spillovers, Homophily, and Selection into Treatment

I establish primitive conditions for unconfoundedness in a coherent model that features heterogeneous treatment effects, spillovers, selection-on-observables, and network formation. I identify average partial effects under minimal exchangeability conditions. If social interactions are also anonymous, I derive a three-dimensional network propensity score, characterize its support conditions, relate it to recent work on network pseudo-metrics, and study extensions. I propose a two-step semiparametric estimator for a random coefficients model which is consistent and asymptotically normal as the number and size of the networks grows. I apply my estimator to a political participation intervention Uganda and a microfinance application in India.

==> figures/bias_stylizedexample.tex <==
% Created by tikzDevice version 0.12 on 2020-09-30 18:23:03
% !TEX encoding = UTF-8 Unicode


==> figures/histrogrampscore.tex <==
% Created by tikzDevice version 0.12 on 2020-02-12 15:23:30
% !TEX encoding = UTF-8 Unicode


==> proofextensions.tex <==
%!TEX root = ./main.tex

\subsection{Proofs Generalized Network Propensity Score}



\begin{proof}[Proof of Corollary \ref{cor:repeatedmeasurements} (\nameref{cor:repeatedmeasurements})]
	If \nameref{assumptxt:independence} holds, then we can apply Lemma \ref{lem:egocentric_factorization} to show that	
	\[
	\mathbb{P}(D_g,G_{ig} \mid V_{ig}) = \mathbb{P}(D_{ig} \mid V_{ig}) \prod_{j\ne i}^{N_g} \mathbb{P}(G_{ijg} \mid V_{ig})  \prod_{j\ne i}^{N_g} \mathbb{P}(D_{jg} \mid V_{ig},G_{ijg}) 
	\]
	If the matching function and unobserved heterogeneity
	\begin{align*}
	\mathbb{P}(G_{ijg} \mid V_{ig} = v) &= \int \prod_{k} p_{\ell \times \ell}(v,v^*)^{G_{ijgk}} (1-p_{\ell \times \ell}(v,v^*))^{1-G_{ijgk}} \ dF(v^* \mid \Psi) \\
	&= \int p_{\ell \times \ell}(v,v^*)^{L_{ijg}} (1-p_{\ell \times \ell}(v,v^*))^{K-L_{ijg}} \ dF(v^* \mid \Psi)
	\end{align*}
	Let $\Delta_L \in \{0,\ldots,K\}$ denote a specific realization of links $G_{ijg}$. The probability of the vector of individual links is completely determined by $\Delta_{L}$, the pairwise link probability $p_{l \times l}$ and the measure $F(\cdot \mid \Psi)$. The latter functions are common across $j \ne i$, so the product of the probability can be established based on the individual count of $\Delta_L$ . Consequently
	\[
	\prod_{j \ne i}\mathbb{P}(G_{ijg} \mid V_{ig}) = H_L(\mu_{ig}(\Delta_{L}),V_{ig})
	\]
	let $\mu_{ig}(\Delta_L,d)$ denote the empirical count of pairwise connections $G_{ijg}$ that have a specific realization of network measures $\Delta_L$ and have a specific treatment status $d$, with corresponding CDF $\mu_{ig}(\Delta_L,d)$. Following the proof of Theorem \ref{thm:weightedcontrolvariable},
	\begin{align*}
	\mathbb{P}(D_{ig}\mid V_{ig})\prod_{j\ne i}^{N_g} \mathbb{P}(D_{jg} \mid V_{ig},G_{ijg}) &= \mathbb{P}(D_{ig};V_{ig})\prod_{(\Delta_L,d)\in \{0,\ldots,K\}\times \{0,1\}} \mathbb{P}(d \mid V_{ig},\Delta_L)^{\mu(G_{ig};\Delta_L,d)}
	\end{align*}
	Since $\mathbb{P}(D_{ig})$ is a Bernoulli with parameter $p_d(V_{ig})$ and $\mathbb{P}(d \mid V_{ig},\Delta_L)$ similarly describes a Bernoulli variable with probability $p_f^L(V_{ig},\Delta_L)$ then we can express the joint-probability concisely in terms of functions $H_D$ and $\widetilde{H}_D$ as
	\begin{align*}
	\mathbb{P}(D_{ig}\mid V_{ig})\prod_{j\ne i}^{N_g} \mathbb{P}(D_{jg} \mid V_{ig},G_{ijg}) &= H_D(D_{ig},\mu(G_{ig};\Delta_L,d),p_d(V_{ig},p_f^L(V_{ig},L))) \\
	&\equiv \widetilde{H}_D(D_{ig},\mu_{ig}(\Delta_L,d),V_{ig})
	\end{align*}
	Consequently we can factor the conditional likelihood in terms of two distinct components.
	\[
	\mathbb{P}(D_g,G_{ig} \mid V_{ig}) = \widetilde{H}_D(D_{ig},\mu_{ig}(\Delta_L,d),V_{ig}) \cdot H_L(\mu_{ig}(\Delta_L),V_{ig})
	\]
	Using similar arguments as Theorem \ref{thm:weightedcontrolvariable},
	\[
	\mathbb{P}(D_{ig},\mu_{ig}(\Delta_L,d) \mid V_{ig},\mu_{ig}(\Delta_L)) \propto \widetilde{H}_D(D_{ig},\mu_{ig}(\Delta_L,d),V_{ig})
	\]
	The proportionality constants depends on counts of the permutations of $(D_g,G_{ig})$ that rationalize $(D_{ig},\mu_{ig}(\Delta_L,d),\mu_{ig}(\Delta_L))$, which does not depend on $V_{ig}$. Therefore, the conditional distribution can be parametrized in terms of $(p_d(V_{ig}),p_f^{L}(V_{ig}),\mu_{ig}(\Delta_L))$ and hence
	\begin{equation}
	(D_{ig},\mu_{ig}(\Delta_L,d),\mu_{ig}(\Delta_L)) \ \indep \ V_{ig} \mid (p_d(V_{ig}),p_f^{L}(V_{ig}),\mu_{ig}(\Delta_L)) 
	\label{eq:proofcondind_repeatmeasures}
	\end{equation}
	By assumption, the function $\omega(G_{ijg})$ is invariant to the order of its arguments, which means that it has to be a function of the total number of reported link between $\{ig\}$ and $\{jg\}$. We simply write this as $\omega^*(\Delta_L)$.
	\begin{align*}
	T_{ig}^{\omega} = \sum_{j \ne i} \omega(G_{ijg}) D_{jg} &= \sum_{j \ne i} \sum_{(\Delta_L,d) \in \{0,\ldots,K\}\times \{0,1\}} \mathbbm{1}\{ (L_{ijg},D_{jg}) = (\Delta_L,d) \} \omega^*(\Delta_L) d \\
	&= \sum_{(\Delta_L,d) \in \{0,\ldots,K\}\times \{0,1\}} \sum_{j \ne i}  \mathbbm{1}\{ (L_{ijg},D_{jg}) = (\Delta,d) \} \omega^*(\Delta_L) d \\
	&= \sum_{(\Delta_L,d) \in \{0,\ldots,K\}\times \{0,1\}} \mu_{ig}(\Delta_L,d)\omega^*(\Delta_L) d
	\end{align*}
	Therefore $T_{ig}$ is measurable with respect to $\mu_{ig}(\Delta_L,d)$. We can use an analogous property to show that $L_{ig}$ is $\mu_{ig}(\Delta_L)-$measurable. By \nameref{assumptxt:weightedinteractions}, \eqref{eq:proofcondind_repeatmeasures} and the decomposition property,
	\[
	X_{ig} \ \indep \ V_{ig} \mid (p_d(V_{ig}),p_f^{L}(V_{ig}),\mu_{ig}(\Delta_L))
	\]
\end{proof}


==> proofsminorlemmas.tex <==
%!TEX root = ./main.tex

\section{Minor Proofs}


\begin{lem}[Clearing]
	Under Assumption \nameref{assumptxt:independence}, $\ p_{nf}(w,a) = \frac{p_D - p_\ell(w,a)p_f(w,a)}{1-p_\ell(w,a)}$.
	\label{lem:equilibriumnonfriends}
\end{lem}

\begin{proof}[Proof of Lemma \ref{lem:equilibriumnonfriends} (Clearing)]
	By Assumption \nameref{assumptxt:independence}, 
	\[
	(W_{ig},A_{ig},\eta_{ig},\varepsilon_{ig}) \ \indep (W_{jg},A_{jg},\eta_{jg},\varepsilon_{jg}) \mid \Psi_g
	\]
	The decomposition axiom implies that $(W_{ig},A_{ig}) \ \indep \ (W_{jg},\eta_{jg})$. Let $p_D \equiv \mathbb{P}(D_{ig} = 1)$ be the unconditional probability that an individual participates in the program. Then
	\begin{equation}
	\begin{alignedat}{3}
	&\mathbb{P}_{\{ D_{jg} \mid W_{ig},A_{ig}\}}(D_{jg} = 1 \mid w,a,\Psi) \\
	&= \int h(w^*,\eta^*) \ dF_{\{W_{jg},\eta_{jg} \mid W_{ig},A_{ig}\}}(w^*,\eta^* \mid w,a,\Psi) &\qquad& \text{($D_{jg} = h(\cdot)$)}\\
	&= \int h(w^*,\eta^*) \ dF_{\{W_{jg},\eta_{jg} \}}(w^*,\eta^*\mid\Psi) && \text{(Independence)} \\
	&= \mathbb{P}(D_{jg} = 1) = p_D &&\text{(Definition $p_D$)}.
	\label{eq:uncond_pD}
	\end{alignedat}
	\end{equation}
	On the other hand, by the law of iterated expectations,
	\begin{equation}
	\mathbb{P}_{\{ D_{jg} \mid W_{ig},A_{ig}\}}(D_{jg} = 1 \mid w,a,\Psi) = p_\ell(w,a)p_f(w,a) + (1-p_\ell)p_{nf}(w,a).
	\label{eq:uncond_iteratedexpectations}
	\end{equation}
	This says that the probability that somebody forms a link is equal to an average of the functions $(p_f(w,a),p_{nf}(w,a))$, the participation probabilities of potential friends / non-friends, weighted by the probability of forming a link. By combining Equations \eqref{eq:uncond_pD} and \eqref{eq:uncond_iteratedexpectations} and rearranging the expression, we find that
	\[
	p_{nf}(w,a) = \frac{p_D - p_\ell(w,a)p_f(w,a)}{1-p_\ell(w,a)}.
	\]
\end{proof}

\begin{lem}
	Suppose that $(X_1,X_2,Y)$ are two random variables such that $X_1 \mid Y \sim Binomial(p_1,Y)$, $X_2 \mid Y \sim Binomial(p_2, Y)$ and $Y \sim Poisson(p_\ell)$, with $p_1,p_2 \in [0,1]$ and $p_\ell < [0,\infty)$. Define the total variation norm, $d_{TV}$ as,
	\[
	d_{TV} \equiv \sum_{x,y \in \mathbb{Z}_{+}^2} \Vert \ p_{X_1,Y}(x,y)- p_{X_2,Y}(x,y) \ \Vert.
	\]
	Then $d_{TV} \le 2 \max\{ 1 - (1-\Vert p_2 - p_1 \Vert )^{p_\ell}, p_\ell \Vert p_2 - p_1 \Vert \}$.
	\label{lem:tv_poissonbinomhier}
\end{lem}

\begin{proof}
		\begin{equation}
	\begin{alignedat}{2}
	d_{TV} &=  \sum_{x,y \mathbb{Z}_{+}^2} \Vert p_{X_1 \mid Y}(x,y)p_Y(y) - p_{X_2 \mid Y}(x,y)p_Y(y) \Vert  &\quad \text{(Bayes' Rule)}\\
&= \sum_{y \in \mathbb{Z}_+} p_Y(y) \underbrace{\sum_{x \in \mathbb{Z}_+} \Vert p_{X_1 \mid Y}(x,y) - p_{X_2 \mid Y}(x,y)\Vert}_{(A)} &\quad \text{(Factorize Terms)}
	\label{eq:tv_poissbinomhier}
	\end{alignedat}
	\end{equation}
    The inner sum in \eqref{eq:tv_poissbinomhier} is the total variation norm between two binomial random variables with parameters $(p_1,p_2)$, respectively. If $p_2 \in (0,1)$, then we can use Theorem 1 and Lemma 2 in \citet{ehm1991binomial} to bound the inner sum by $y \Vert p_1 - p_2\Vert ^2$, which is weakly less than $2 y \Vert p_1 - p_2 \Vert$ since $\Vert p_1 - p_2 \Vert \in [0,1]$. In this case, the total variation norm is bounded by $2 \sum_{y \in \mathbb{Z}_+} p_Y(y) y \Vert p_1 - p_2 \Vert$, which is equal to $2 p_\ell  \Vert p_1 - p_2 \Vert $ since $Y$ is a Poisson random variable with rate $p_\ell$.
	
	If $p_2 = 0$, the term (A) in \eqref{eq:tv_poissbinomhier} is the total variation between a binomial random variable $(p_1)$ and a degenerate random variable with mass at zero. That means that $p_{X_2 \mid Y}(x,y)$ is zero for all $y > 0$ and consequently $\Vert p_{X_1 \mid Y}(0,y) - p_{X_2 \mid Y}(0,y)\Vert = p_{X_1 \mid Y}(0,y)$ in that range. We can just add and subtract the term $p_{X_1 \mid Y}(0,y)$ to show that (A) is equal to
 \begin{equation}
\begin{alignedat}{2}
&\left(\sum_{x \in \mathbb{Z}_{+}} p_{X_1 \mid Y}(x,y)\right) - p_{X_1 \mid Y}(0,y) +  \Vert p_{X_1 \mid Y}(0,y) - p_{X_2 \mid Y}(0,y)\Vert \\
&= 1 - (1-p_1)^{y} + \Vert (1-p_1)^y - 1 \Vert &\quad\text{(Binomial Probability)}\\
&= 2 (1 - (1-p_1)^{y})  &\quad \text{(Since $p_1 \in [0,1]$)}
\label{eq:tv_poissbinomhier_corner0}
\end{alignedat}
\end{equation}
The last expression is a concave function of $y$ over $y \ge 0$. We can then use Jensen's inequality to show that
\begin{equation}
\sum_{x \in \mathbb{Z}_+} p_Y(y) (1 - (1-p_1)^{y}) \ \le \ 1 - (1-p_1)^{\sum_{x \in \mathbb{Z}_+} y \ p_Y(y)}
\label{eq:tv_poissbinomhier_corner0_jensen}
\end{equation}
Since $Y$ is distributed as a Poisson random variable $\sum_{x \in \mathbb{Z}_+} y \ p_Y(y) = p_\ell$. Thus when $p_2 = 0$, $\Vert p_1 - p_2 \Vert = p_1$ and the total variation norm can be bounded by $ 1 - (1-\Vert p_1 - p_2 \Vert )^{p_\ell}$.

Similarly, when $p_2 = 1$, we can show that $(A)$ in \eqref{eq:tv_poissbinomhier} is equal to
 \begin{equation}
\begin{alignedat}{2}
&\left(\sum_{x \in \mathbb{Z}_{+}} p_{X_1 \mid Y}(x,y)\right) - p_{X_1 \mid Y}(y,y) +  \Vert p_{X_1 \mid Y}(y,y) - p_{X_2 \mid Y}(y,y)\Vert \\
&= 1 - p_1^y + \Vert p_1^y - 1 \Vert &\quad\text{(Binomial Probability)}\\
&= 2(1 - p_1^y ) &\quad \text{(Since $p_1 \in [0,1]$)}\\
&= 2 (1 - (1-\Vert p_1 - p_2\Vert))^{y}  &\quad \text{(For $p_2 = 0$)}
\label{eq:tv_poissbinomhier_corner1}
\end{alignedat}
\end{equation}
By using Jensen's inequality again we can show that when $p_2 = 1$, the total variation norm is bounded by $1 - (1-\Vert p_1 - p_2 \Vert )^{p_\ell}$. To compute a uniform bound over the range $p_2 \in [0,1]$ it suffices to compute the maximum across bounds
\[
d_{TV} \le 2 \max\{ 1 - (1-\Vert p_2 - p_1 \Vert )^{p_\ell}, p_\ell \Vert p_2 - p_1 \Vert \}
\]

\end{proof}

==> tables/outputfigures/bias_stylizedexample.tex <==
% Created by tikzDevice version 0.12 on 2020-11-04 19:28:38
% !TEX encoding = UTF-8 Unicode


==> tables/outputfigures/histrogrampscore.tex <==
% Created by tikzDevice version 0.12 on 2020-02-12 15:23:30
% !TEX encoding = UTF-8 Unicode


==> tables/outputfigures/networksaturation_stylizedexample.tex <==
% Created by tikzDevice version 0.12 on 2020-11-04 19:28:42
% !TEX encoding = UTF-8 Unicode


==> tables/outputfigures/randomsaturation_stylizedexample.tex <==
% Created by tikzDevice version 0.12 on 2020-11-04 19:28:40
% !TEX encoding = UTF-8 Unicode


==> tables/outputunweighted/y.tex <==
names,coef,se,tstat
ones,-3.024,0.385,-7.8545454545454545
rooftype2,0.167,0.243,0.6872427983539096
rooftype3,0.522,0.192,2.71875
rooftype4,0.443,0.19,2.331578947368421
room_no,0.072,0.047,1.5319148936170213
delectr_private,0.287,0.169,1.6982248520710057
dlatrineaccess,0.254,0.127,2
downrent_agg_rent,-0.629,0.259,-2.4285714285714284
dcaste_obc,-0.455,0.161,-2.8260869565217392
dcaste_scst,-0.428,0.212,-2.018867924528302
fracfriends,13.803,2.955,4.671065989847716
t,-0.008,0.045,-0.17777777777777778
sigma1,-0.309,0.528,-0.5852272727272727
ones,-1.667,0.251,-6.6414342629482075
rooftype2,-0.069,0.103,-0.6699029126213594
rooftype3,0.098,0.119,0.823529411764706
rooftype4,-0.111,0.096,-1.15625
room_no,0.041,0.023,1.782608695652174
delectr_private,-0.022,0.059,-0.3728813559322034
dlatrineaccess,0.12,0.078,1.5384615384615383
downrent_agg_rent,-0.067,0.122,-0.5491803278688525
dcaste_obc,-0.291,0.09,-3.2333333333333334
dcaste_scst,-0.423,0.132,-3.204545454545454
fracfriends,6.268,2.882,2.1748785565579456
t,-0.02,0.039,-0.5128205128205129
sigma2,0.399,0.153,2.607843137254902
sigma3,-5.887,2.223,-2.6482231219073324
beta0,0.158,0.009,17.555555555555557
beta1,0.118,0.018,6.555555555555555
beta2,0.001,0.064,0.015625


==> tables/table2_summary.tex <==
 \begin{tabular}{lccc}  \hline &  Full Data & Non Leaders & Leaders \\ \  &  (N = 9,598) &  (N = 8,441) &  (N = 1,157)\\ \ \bf{Caste} & ~ & ~ & ~\\ \ ~~ General & 10 \% & 9 \% & 17 \%\\ \ ~~ Minority & 3 \% & 3 \% & 2 \%\\ \ ~~ OBC & 42 \% & 42 \% & 45 \%\\ \ ~~ Scheduled Caste & 23 \% & 24 \% & 18 \%\\ \ ~~ Scheduled Tribe & 4 \% & 4 \% & 4 \%\\ \ ~~ Not reported & 17 \% & 18 \% & 14 \%\\ \ \bf{Religion} & ~ & ~ & ~\\ \ ~~ Hinduism & 95 \% & 95 \% & 96 \%\\ \ ~~ Islam & 5 \% & 5 \% & 4 \%\\ \ ~~ Christianity & 0.09 \% & 0.09 \% & 0.09 \%\\ \ \bf{Number of Connections} & ~ & ~ & ~\\ \ ~~ None & 5 \% & 5 \% & 1 \%\\ \ ~~ At least one one & 95 \% & 95 \% & 99 \%\\ \ ~~ Mean & 9.25 & 8.77 & 12.72\\ \ ~~ Standard Deviation & 7.57 & 7.17 & 9.32\\ \hline \ \end{tabular}


==> tables/table_mainspecification.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Thu, May 30, 2019 - 7:17:14 PM
\begin{tabular}{@{\extracolsep{5pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
\\[-1.8ex] & DR\_Pool & DR\_Corr & OLS\_No\_covar & OLS\_Covar \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 Direct\_Effect & 0.113$^{***}$ & 0.108$^{***}$ & 0.082$^{***}$ & 0.090$^{***}$ \\ 
  & (0.027) & (0.027) & (0.025) & (0.025) \\ 
  & & & & \\ 
 Indirect\_Effect & 0.094 & 0.090 & 0.0002 & 0.021 \\ 
  & (0.059) & (0.057) & (0.036) & (0.031) \\ 
  & & & & \\ 
 Interaction & $-$0.212 & $-$0.178 & $-$0.120 & $-$0.104 \\ 
  & (0.136) & (0.130) & (0.102) & (0.100) \\ 
  & & & & \\ 
 Constant & 0.158$^{***}$ & 0.159$^{***}$ & 0.177$^{***}$ & $-$0.013 \\ 
  & (0.012) & (0.012) & (0.012) & (0.059) \\ 
  & & & & \\ 
\hline \\[-1.8ex] 
Observations & 9,116 & 9,116 & 9,116 & 9,116 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 


==> tables/table_mainspecification_eigenvectorplusnumfriends.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Sat, Mar 02, 2019 - 12:14:58 PM
\begin{tabular}{@{\extracolsep{5pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
\\[-1.8ex] & Intercept & Direct\_Effect & Indirect\_Effect & Alpha \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 IPW\_Pool & 0.156$^{***}$ & 0.086$^{***}$ & 0.136$^{**}$ &  \\ 
  & (0.015) & (0.014) & (0.067) &  \\ 
  & & & & \\ 
 DR\_Pool & 0.160$^{***}$ & 0.088$^{***}$ & 0.077 &  \\ 
  & (0.014) & (0.014) & (0.058) &  \\ 
  & & & & \\ 
 IPW\_Corr & 0.161$^{***}$ & 0.086$^{***}$ & 0.107 &  \\ 
  & (0.015) & (0.014) & (0.066) &  \\ 
  & & & & \\ 
 DR\_Corr & 0.161$^{***}$ & 0.088$^{***}$ & 0.075 &  \\ 
  & (0.014) & (0.014) & (0.057) &  \\ 
  & & & & \\ 
 OLS\_No\_covar & 0.179$^{***}$ & 0.060$^{***}$ & $-$0.013 &  \\ 
  & (0.013) & (0.012) & (0.033) &  \\ 
  & & & & \\ 
 OLS\_Covar & 0.080$^{*}$ & 0.071$^{***}$ & 0.003 &  \\ 
  & (0.042) & (0.013) & (0.031) &  \\ 
  & & & & \\ 
 LIM\_No\_Cov & 0.092$^{***}$ & 0.058$^{***}$ & $-$0.010 & 0.432$^{***}$ \\ 
  & (0.009) & (0.011) & (0.025) & (0.033) \\ 
  & & & & \\ 
 LIM\_Cov & 0.005 & 0.064$^{***}$ & 0.0005 & 0.379$^{***}$ \\ 
  & (0.031) & (0.012) & (0.025) & (0.032) \\ 
  & & & & \\ 
\hline \\[-1.8ex] 
Observations & 9,122 & 9,122 & 9,122 & 9,122 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 


==> tables/tablefscorepprobit.tex <==
 \begin{tabular}{lcccccc} \hline & \multicolumn{2}{c}{Model (1)}& \multicolumn{2}{c}{Model (2)}& \multicolumn{2}{c}{Model (3)} \\&  Coef. & S.E. &  Coef. & S.E. &  Coef. & S.E.\\ \hline \\\   \ \bf{Roof Type (Other)} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ Thatch & -0.06 & (0.17) & -0.06 & (0.17) & -0.08 & (0.17)\\ \ ~~ Tile & 0.06 & (0.09) & 0.06 & (0.09) & 0.05 & (0.09)\\ \ ~~ Stone & 0.18*** & (0.09) & 0.18*** & (0.09) & 0.18*** & (0.09)\\ \ ~~ Sheet & 0.15 & (0.09) & 0.15 & (0.09) & 0.15 & (0.09)\\ \ ~~ RCC & 0.19* & (0.1) & 0.19* & (0.1) & 0.19* & (0.1)\\ \ \bf{Electricity (Yes, Government)} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ Yes, Private & -0.09*** & (0.04) & -0.09*** & (0.04) & -0.09*** & (0.04)\\ \ ~~ No & -0.13 & (0.09) & -0.13 & (0.09) & -0.12 & (0.09)\\ \ \bf{Latrine (Owned)} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ Common & 0.09 & (0.24) & 0.09 & (0.24) & 0.08 & (0.24)\\ \ ~~ None & -0.19*** & (0.04) & -0.19*** & (0.04) & -0.18*** & (0.04)\\ \ \bf{Residence (Owned)} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ Owned but shared & 0.12 & (0.18) & 0.12 & (0.18) & 0.12 & (0.18)\\ \ ~~ Rented & -0.25*** & (0.1) & -0.25*** & (0.1) & -0.24*** & (0.1)\\ \ ~~ Leased & 0.19 & (0.43) & 0.19 & (0.43) & 0.22 & (0.43)\\ \ ~~ Given by government & -0.05 & (0.1) & -0.06 & (0.1) & -0.05 & (0.1)\\ \ ~~ Other & -3.49 & (59.21) & -3.49 & (59.33) & -3.47 & (59.71)\\ \ \bf{Religion (Hinduism)} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ Islam & -0.08 & (0.14) & -0.08 & (0.14) & -0.06 & (0.14)\\ \ ~~ Christianity & -0.01 & (0.57) & -0.01 & (0.57) & 0 & (0.56)\\ \ \bf{Caste (Not Reported)} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ OBC & -0.06 & (0.06) & -0.06 & (0.06) & -0.03 & (0.06)\\ \ ~~ Schedule Caste & -0.1 & (0.07) & -0.1 & (0.07) & -0.09 & (0.07)\\ \ ~~ Minority & -0.08 & (0.19) & -0.08 & (0.19) & -0.04 & (0.19)\\ \ ~~ General & 0.17*** & (0.08) & 0.17*** & (0.08) & 0.22*** & (0.08)\\ \ ~~ Schedule Tribe & -0.1 & (0.11) & -0.1 & (0.11) & -0.06 & (0.11)\\ \ \bf{Other Variables} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ No. Rooms & 0.04*** & (0.01) & 0.04*** & (0.02) & 0.04*** & (0.01)\\ \ ~~ Number of Friends & 0.03*** & (0) & 0.03*** & (0) & 0.01*** & (0)\\ \ ~~ Months since Program Start &  &  & 0 & (0.02) & 0 & (0.01)\\ \ ~~ Eigenvector Centrality &  &  &  &  & 2.66*** & (0.7)\\ \ \bf{Random Effects Coefficient} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ Unobserved heterogeneity & 0.13 &  & 0.13 &  & 0.12 & \\ \hline \ \end{tabular}


==> tables/tablepooledprobit.tex <==
 \begin{tabular}{lcccccc} \hline & \multicolumn{2}{c}{Model (1)}& \multicolumn{2}{c}{Model (2)}& \multicolumn{2}{c}{Model (3)}\\&  Coef. & S.E. &  Coef. & S.E. &  Coef. & S.E.\\ \hline \\\              \ \bf{Roof Type (Other)} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ Thatch & -0.08 & (0.17) & -0.08 & (0.17) & -0.09 & (0.17)\\ \ ~~ Tile & 0.03 & (0.09) & 0.03 & (0.09) & 0.03 & (0.09)\\ \ ~~ Stone & 0.18*** & (0.09) & 0.18*** & (0.09) & 0.17* & (0.09)\\ \ ~~ Sheet & 0.11 & (0.09) & 0.11 & (0.09) & 0.12 & (0.09)\\ \ ~~ RCC & 0.16* & (0.1) & 0.16 & (0.1) & 0.16 & (0.1)\\ \ \bf{Electricity (Yes, Government)} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ Yes, Private & -0.07 & (0.04) & -0.07 & (0.04) & -0.07 & (0.04)\\ \ ~~ No & -0.13 & (0.08) & -0.13 & (0.08) & -0.12 & (0.08)\\ \ \bf{Latrine (Owned)} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ Common & 0.06 & (0.24) & 0.06 & (0.24) & 0.06 & (0.24)\\ \ ~~ None & -0.19*** & (0.04) & -0.19*** & (0.04) & -0.18*** & (0.04)\\ \ \bf{Residence (Owned)} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ Owned but shared & 0.12 & (0.18) & 0.12 & (0.18) & 0.12 & (0.18)\\ \ ~~ Rented & -0.25*** & (0.09) & -0.25*** & (0.09) & -0.25*** & (0.09)\\ \ ~~ Leased & 0.21 & (0.43) & 0.21 & (0.43) & 0.25 & (0.43)\\ \ ~~ Given by government & -0.06 & (0.1) & -0.06 & (0.1) & -0.05 & (0.1)\\ \ ~~ Other & -3.35 & (40.95) & -3.35 & (40.95) & -3.33 & (40.98)\\ \ \bf{Religion (Hinduism)} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ Islam & -0.05 & (0.13) & -0.05 & (0.13) & -0.03 & (0.13)\\ \ ~~ Christianity & 0.02 & (0.57) & 0.02 & (0.57) & 0.03 & (0.57)\\ \ \bf{Caste (General)} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ OBC & -0.05 & (0.04) & -0.05 & (0.05) & -0.02 & (0.05)\\ \ ~~ Schedule Caste & -0.09 & (0.06) & -0.09 & (0.06) & -0.08 & (0.06)\\ \ ~~ Schedule Tribe & -0.11 & (0.1) & -0.11 & (0.1) & -0.05 & (0.1)\\ \ ~~ Minority & -0.07 & (0.17) & -0.07 & (0.17) & -0.04 & (0.17)\\ \ ~~ General & 0.18*** & (0.06) & 0.18*** & (0.06) & 0.24*** & (0.07)\\ \ \bf{Other Variables} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ No. Rooms & 0.04*** & (0.01) & 0.04*** & (0.01) & 0.04*** & (0.01)\\ \ ~~ Number of Friends & 0.03*** & (0) & 0.03*** & (0) & 0.01*** & (0)\\ \ ~~ Months since Program Start &  &  & 0 & (0.01) & 0 & (0.01)\\ \ ~~ Eigenvector Centrality &  &  &  &  & 2.96*** & (0.67)\\ \hline \ \end{tabular}


==> tables/tableprobit.tex <==

\begin{tabular}{l c c c c }
\hline
 & Model 1 & Model 2 & Model 3 & Model 4 \\
\hline
(Intercept)                             & $-1.14 \; (0.10)^{***}$ & $-1.43 \; (0.11)^{***}$ & $-1.14 \; (0.11)^{***}$ & $-1.44 \; (0.11)^{***}$ \\
rooftype1                               & $-0.10 \; (0.17)$       & $-0.13 \; (0.17)$       & $-0.09 \; (0.17)$       & $-0.12 \; (0.17)$       \\
rooftype2                               & $0.01 \; (0.09)$        & $0.01 \; (0.09)$        & $0.03 \; (0.09)$        & $0.03 \; (0.09)$        \\
rooftype3                               & $0.15 \; (0.09)$        & $0.14 \; (0.09)$        & $0.16 \; (0.09)$        & $0.16 \; (0.09)$        \\
rooftype4                               & $0.08 \; (0.09)$        & $0.11 \; (0.09)$        & $0.11 \; (0.09)$        & $0.14 \; (0.09)$        \\
rooftype5                               & $0.15 \; (0.10)$        & $0.15 \; (0.10)$        & $0.17 \; (0.10)$        & $0.18 \; (0.10)$        \\
room\_no                                & $0.07 \; (0.01)^{***}$  & $0.04 \; (0.01)^{**}$   & $0.07 \; (0.01)^{***}$  & $0.04 \; (0.01)^{**}$   \\
bed\_no                                 & $0.00 \; (0.01)$        & $-0.00 \; (0.01)$       & $0.01 \; (0.01)$        & $-0.00 \; (0.01)$       \\
as.factor(electricity)2                 & $-0.09 \; (0.04)^{*}$   & $-0.07 \; (0.04)$       & $-0.11 \; (0.04)^{*}$   & $-0.09 \; (0.04)^{*}$   \\
as.factor(electricity)3                 & $-0.21 \; (0.08)^{*}$   & $-0.14 \; (0.08)$       & $-0.21 \; (0.08)^{**}$  & $-0.15 \; (0.08)$       \\
latrine                                 & $-0.10 \; (0.02)^{***}$ & $-0.08 \; (0.02)^{***}$ & $-0.10 \; (0.02)^{***}$ & $-0.08 \; (0.02)^{***}$ \\
as\_factor(ownrent)OWNED BUT SHARED     & $0.15 \; (0.16)$        & $0.16 \; (0.17)$        & $0.15 \; (0.17)$        & $0.17 \; (0.17)$        \\
as\_factor(ownrent)RENTED               & $-0.32 \; (0.09)^{***}$ & $-0.25 \; (0.09)^{**}$  & $-0.31 \; (0.09)^{***}$ & $-0.25 \; (0.09)^{**}$  \\
as\_factor(ownrent)LEASED               & $0.04 \; (0.41)$        & $0.16 \; (0.41)$        & $0.02 \; (0.41)$        & $0.14 \; (0.41)$        \\
as\_factor(ownrent)GIVEN BY GOVERNMENT  & $-0.03 \; (0.09)$       & $-0.03 \; (0.10)$       & $-0.03 \; (0.10)$       & $-0.04 \; (0.10)$       \\
as\_factor(ownrent)6                    & $-3.50 \; (40.87)$      & $-3.32 \; (40.94)$      & $-4.23 \; (400.09)$     & $-4.05 \; (395.68)$     \\
as\_factor(hohreligion)ISLAM            & $-0.08 \; (0.13)$       & $-0.01 \; (0.13)$       & $-0.11 \; (0.13)$       & $-0.02 \; (0.13)$       \\
as\_factor(hohreligion)CHRISTIANITY     & $0.02 \; (0.57)$        & $0.05 \; (0.57)$        & $-0.00 \; (0.57)$       & $0.03 \; (0.57)$        \\
as\_factor(castesubcaste)OBC            & $-0.02 \; (0.04)$       & $0.02 \; (0.04)$        & $-0.03 \; (0.06)$       & $0.02 \; (0.06)$        \\
as\_factor(castesubcaste)SCHEDULE CASTE & $-0.06 \; (0.05)$       & $-0.06 \; (0.05)$       & $-0.07 \; (0.07)$       & $-0.06 \; (0.07)$       \\
as\_factor(castesubcaste)MINORITY       & $-0.07 \; (0.17)$       & $-0.02 \; (0.17)$       & $-0.08 \; (0.18)$       & $-0.01 \; (0.18)$       \\
as\_factor(castesubcaste)GENERAL        & $0.22 \; (0.06)^{***}$  & $0.30 \; (0.06)^{***}$  & $0.21 \; (0.07)^{**}$   & $0.29 \; (0.07)^{***}$  \\
as\_factor(castesubcaste)SCHEDULE TRIBE & $-0.04 \; (0.10)$       & $0.01 \; (0.10)$        & $-0.05 \; (0.11)$       & $0.01 \; (0.11)$        \\
eigenvector                             &                         & $4.76 \; (0.35)^{***}$  &                         & $4.80 \; (0.35)^{***}$  \\
sigma                                   &                         &                         & $0.16 \; (0.04)^{***}$  & $0.15 \; (0.04)^{***}$  \\
\hline
AIC                                     & 6885.45                 & 6705.34                 &                         &                         \\
BIC                                     & 7050.33                 & 6877.39                 &                         &                         \\
Log Likelihood                          & -3419.72                & -3328.67                &                         &                         \\
Deviance                                & 6839.45                 & 6657.34                 &                         &                         \\
Num. obs.                               & 9594                    & 9594                    & 9594                    & 9594                    \\
Log-Likelihood                          &                         &                         & -3413.84                & -3323.34                \\
\hline
\multicolumn{5}{l}{\scriptsize{The coefficients are presented with standard errors in parenthesis.}}
\end{tabular}


==> tables/tablereprobit.tex <==
 \begin{tabular}{lcccccc} \hline & \multicolumn{2}{c}{Model (1)}& \multicolumn{2}{c}{Model (2)}& \multicolumn{2}{c}{Model (3)} \\&  Coef. & S.E. &  Coef. & S.E. &  Coef. & S.E.\\ \hline \\\   \ \bf{Roof Type (Other)} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ Thatch & -0.06 & (0.17) & -0.06 & (0.17) & -0.08 & (0.17)\\ \ ~~ Tile & 0.06 & (0.09) & 0.06 & (0.09) & 0.05 & (0.09)\\ \ ~~ Stone & 0.18*** & (0.09) & 0.18*** & (0.09) & 0.18*** & (0.09)\\ \ ~~ Sheet & 0.15 & (0.09) & 0.15 & (0.09) & 0.15 & (0.09)\\ \ ~~ RCC & 0.19* & (0.1) & 0.19* & (0.1) & 0.19* & (0.1)\\ \ \bf{Electricity (Yes, Government)} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ Yes, Private & -0.09*** & (0.04) & -0.09*** & (0.04) & -0.09*** & (0.04)\\ \ ~~ No & -0.13 & (0.09) & -0.13 & (0.09) & -0.12 & (0.09)\\ \ \bf{Latrine (Owned)} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ Common & 0.09 & (0.24) & 0.09 & (0.24) & 0.08 & (0.24)\\ \ ~~ None & -0.19*** & (0.04) & -0.19*** & (0.04) & -0.18*** & (0.04)\\ \ \bf{Residence (Owned)} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ Owned but shared & 0.12 & (0.18) & 0.12 & (0.18) & 0.12 & (0.18)\\ \ ~~ Rented & -0.25*** & (0.1) & -0.25*** & (0.1) & -0.24*** & (0.1)\\ \ ~~ Leased & 0.19 & (0.43) & 0.19 & (0.43) & 0.22 & (0.43)\\ \ ~~ Given by government & -0.05 & (0.1) & -0.06 & (0.1) & -0.05 & (0.1)\\ \ ~~ Other & -3.49 & (59.21) & -3.49 & (59.33) & -3.47 & (59.71)\\ \ \bf{Religion (Hinduism)} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ Islam & -0.08 & (0.14) & -0.08 & (0.14) & -0.06 & (0.14)\\ \ ~~ Christianity & -0.01 & (0.57) & -0.01 & (0.57) & 0 & (0.56)\\ \ \bf{Caste (Not Reported)} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ OBC & -0.06 & (0.06) & -0.06 & (0.06) & -0.03 & (0.06)\\ \ ~~ Schedule Caste & -0.1 & (0.07) & -0.1 & (0.07) & -0.09 & (0.07)\\ \ ~~ Minority & -0.08 & (0.19) & -0.08 & (0.19) & -0.04 & (0.19)\\ \ ~~ General & 0.17*** & (0.08) & 0.17*** & (0.08) & 0.22*** & (0.08)\\ \ ~~ Schedule Tribe & -0.1 & (0.11) & -0.1 & (0.11) & -0.06 & (0.11)\\ \ \bf{Other Variables} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ No. Rooms & 0.04*** & (0.01) & 0.04*** & (0.02) & 0.04*** & (0.01)\\ \ ~~ Number of Friends & 0.03*** & (0) & 0.03*** & (0) & 0.01*** & (0)\\ \ ~~ Months since Program Start &  &  & 0 & (0.02) & 0 & (0.01)\\ \ ~~ Eigenvector Centrality &  &  &  &  & 2.66*** & (0.7)\\ \ \bf{Random Effects Coefficient} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ Unobserved heterogeneity & 0.13 &  & 0.13 &  & 0.12 & \\ \hline \ \end{tabular}


==> tables/tablesfscoreprobit.tex <==
 \begin{tabular}{lcc} \hline & \multicolumn{2}{c}{Model (1)}\\&  Coef. & S.E.\\ \hline \\\      \ \bf{Roof Type (Other)} & ~ & ~\\ \ ~~ Thatch & -0.19 & (0.11)\\ \ ~~ Tile & -0.13* & (0.08)\\ \ ~~ Stone & -0.03 & (0.07)\\ \ ~~ Sheet & -0.13*** & (0.06)\\ \ ~~ RCC & -0.07 & (0.07)\\ \ \bf{Electricity (Yes, Government)} & ~ & ~\\ \ ~~ Yes, Private & 0.01 & (0.04)\\ \ ~~ No & -0.1* & (0.06)\\ \ \bf{Latrine (Owned)} & ~ & ~\\ \ ~~ Common & -0.08 & (0.13)\\ \ ~~ None & -0.1*** & (0.03)\\ \ \bf{Residence (Owned)} & ~ & ~\\ \ ~~ Owned but shared & 0.11 & (0.16)\\ \ ~~ Rented & 0.06 & (0.09)\\ \ ~~ Leased & 0.14 & (0.32)\\ \ ~~ Given by government & -0.04 & (0.07)\\ \ ~~ Other & -0.36 & (0.65)\\ \ \bf{Religion (Hinduism)} & ~ & ~\\ \ ~~ Islam & 0.17 & (0.16)\\ \ ~~ Christianity & 0.48 & (0.39)\\ \ \bf{Caste (General)} & ~ & ~\\ \ ~~ OBC & -0.26*** & (0.09)\\ \ ~~ Schedule Caste & -0.34*** & (0.11)\\ \ ~~ Schedule Tribe & -0.19* & (0.11)\\ \ ~~ Minority & -0.41* & (0.24)\\ \ ~~ Non-response & -0.1 & (0.13)\\ \ \bf{Other Variables} & ~ & ~\\ \ ~~ No. Rooms & 0 & (0.01)\\ \hline \ \end{tabular}


==> tables/tableslscoreprobit.tex <==
 \begin{tabular}{lcccccc} \hline & \multicolumn{2}{c}{Model (1)}& \multicolumn{2}{c}{Model (2)}& \multicolumn{2}{c}{Model (3)} \\&  Coef. & S.E. &  Coef. & S.E. &  Coef. & S.E.\\ \hline \\\   \ \bf{Roof Type (Other)} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ Thatch & -0.06 & (0.17) & -0.06 & (0.17) & -0.08 & (0.17)\\ \ ~~ Tile & 0.06 & (0.09) & 0.06 & (0.09) & 0.05 & (0.09)\\ \ ~~ Stone & 0.18*** & (0.09) & 0.18*** & (0.09) & 0.18*** & (0.09)\\ \ ~~ Sheet & 0.15 & (0.09) & 0.15 & (0.09) & 0.15 & (0.09)\\ \ ~~ RCC & 0.19* & (0.1) & 0.19* & (0.1) & 0.19* & (0.1)\\ \ \bf{Electricity (Yes, Government)} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ Yes, Private & -0.09*** & (0.04) & -0.09*** & (0.04) & -0.09*** & (0.04)\\ \ ~~ No & -0.13 & (0.09) & -0.13 & (0.09) & -0.12 & (0.09)\\ \ \bf{Latrine (Owned)} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ Common & 0.09 & (0.24) & 0.09 & (0.24) & 0.08 & (0.24)\\ \ ~~ None & -0.19*** & (0.04) & -0.19*** & (0.04) & -0.18*** & (0.04)\\ \ \bf{Residence (Owned)} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ Owned but shared & 0.12 & (0.18) & 0.12 & (0.18) & 0.12 & (0.18)\\ \ ~~ Rented & -0.25*** & (0.1) & -0.25*** & (0.1) & -0.24*** & (0.1)\\ \ ~~ Leased & 0.19 & (0.43) & 0.19 & (0.43) & 0.22 & (0.43)\\ \ ~~ Given by government & -0.05 & (0.1) & -0.06 & (0.1) & -0.05 & (0.1)\\ \ ~~ Other & -3.49 & (59.21) & -3.49 & (59.33) & -3.47 & (59.71)\\ \ \bf{Religion (Hinduism)} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ Islam & -0.08 & (0.14) & -0.08 & (0.14) & -0.06 & (0.14)\\ \ ~~ Christianity & -0.01 & (0.57) & -0.01 & (0.57) & 0 & (0.56)\\ \ \bf{Caste (Not Reported)} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ OBC & -0.06 & (0.06) & -0.06 & (0.06) & -0.03 & (0.06)\\ \ ~~ Schedule Caste & -0.1 & (0.07) & -0.1 & (0.07) & -0.09 & (0.07)\\ \ ~~ Minority & -0.08 & (0.19) & -0.08 & (0.19) & -0.04 & (0.19)\\ \ ~~ General & 0.17*** & (0.08) & 0.17*** & (0.08) & 0.22*** & (0.08)\\ \ ~~ Schedule Tribe & -0.1 & (0.11) & -0.1 & (0.11) & -0.06 & (0.11)\\ \ \bf{Other Variables} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ No. Rooms & 0.04*** & (0.01) & 0.04*** & (0.02) & 0.04*** & (0.01)\\ \ ~~ Number of Friends & 0.03*** & (0) & 0.03*** & (0) & 0.01*** & (0)\\ \ ~~ Months since Program Start &  &  & 0 & (0.02) & 0 & (0.01)\\ \ ~~ Eigenvector Centrality &  &  &  &  & 2.66*** & (0.7)\\ \ \bf{Random Effects Coefficient} & ~ & ~ & ~ & ~ & ~ & ~\\ \ ~~ Unobserved heterogeneity & 0.13 &  & 0.13 &  & 0.12 & \\ \hline \ \end{tabular}

